Stability of NLO Global Analysis and Implications for Hadron Collider Physics

The phenomenology of Standard Model and New Physics at hadron colliders depends critically on results from global QCD analysis for parton distribution functions (PDFs). The accuracy of the standard next-to-leading-order (NLO) global analysis, nominally a few percent, is generally well matched to the expected experimental precision. However, serious questions have been raised recently about the stability of the NLO analysis with respect to certain inputs, including the choice of kinematic cuts on the data sets and the parametrization of the gluon distribution. In this paper, we investigate this stability issue systematically within the CTEQ framework. We find that both the PDFs and their physical predictions are stable, well within the few percent level. Further, we have applied the Lagrange Multiplier method to explore the stability of the predicted cross sections for W production at the Tevatron and the LHC, since W production is often proposed as a standard candle for these colliders. We find the NLO predictions on sigma_W to be stable well within their previously-estimated uncertainty ranges.

==> text/t1 <==
1intro.tex:In recent years, some preliminary next-to-next-leading-order (NNLO) analyses
1intro.tex:The NNLO evolution kernel was also only known approximately at the time of
1intro.tex:All other considerations being equal, a global analysis at NNLO must be
6finale.tex:Tevatron and at the LHC. Further improvement will be possible with a NNLO 
6finale.tex:global QCD analysis. A fully global analysis at NNLO, however, must wait for 
6finale.tex:the completion of the NNLO QCD calculation of all of the relevant hard 
appendix.tex:differ only at NNLO, so \textit{a priori} they are equally valid at NLO.  
appendix.tex:a NNLO term that depends on
stability.cit:%``NNLO parton distributions from deep-inelastic scattering data,''
stability.cit:%``NNLO global parton analysis,''

